Ground state baryons in the flux-tube three-body confinement model using Diffusion Monte Carlo

We make a systematical diffusion Monte Carlo (DMC) calculation for all ground state baryons in two confinement scenarios, the pairwise confinement and the three-body flux-tube confinement. With the baryons as an example, we illustrate a feasible procedure to investigate the few-quark states with possible few-body confinement mechanisms, which can be extended to the multiquark states easily. For each baryon, we extract the mass, mean-square radius, charge radius, and the quark distributions. We use the Jackknife resampling method to estimate the statistical uncertainties of masses to be less than 1 MeV. To determine the baryon charge radii, we include the constituent quark size effect, which is fixed by the experimental and lattice QCD results. Our results show that both two-body and three-body confinement mechanisms can give a good description of the experimental data if the parameters are chosen properly. In the flux-tube confinement, introducing different tension parameters for the baryons and mesons are necessary, specifically, $\sigma_Y= 0.9204 \sigma_{Q\bar{Q}}$. The lesson from the calculation of the nucleon mass with the DMC method is that the improper pre-assignment of the channels may prevent us from obtaining the real ground state. With this experience, we obtain the real ground state (the $\eta_c \eta_c$ threshold with the di-meson configuration) of the $cc\bar{c}\bar{c}$ system with $J^{PC}=0^{++}$ starting from the diquark-antidiquark spin-color channels alone, which is hard to achieve in the variational method and was not obtained in the previous DMC calculations.

==> reply1.tex <==
   Dear Editor,
    \\

    Thank you very much for handling our paper. We are grateful to the
    referee for reading our manuscript (DY13020) so carefully. We thank
    the referee for her/his constructive report. We have followed the
    concerns/comments and revised our manuscript accordingly. We
    sincerely hope that our paper will be published in \textit{Physical Review D}.

    \vspace{0.4cm} Sincerely,

    \vspace{0.4cm}

    ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Yao Ma, Lu Meng, Yan-Ke Chen and Shi-Lin Zhu.\\~\\

    \noindent---------------------------------------------------------------------------------------
    \\ Reply to the Referee and Summary of Changes Made, DY13020\\
    -----------------------------------------------------------------------------------------\\

Since the referee's concerns and suggestions are very reasonable, we have followed his/her suggestions item by item and revised the draft accordingly. The changes  are shown in \textcolor{red}{RED} in the draft following this letter. In this letter, we first quote the referee's question/comment, then list our reply. The referee can go to specific changes by using the labels e.g. \cref{Jackknife} with hyperlinks.  \\

{\bf Question:}\textit{ In the first paragraph of Sec. IV, authors state that they average the values of energy in the last 5000 steps of evolution and uncertainty
reduces to $1/\sqrt{5000}$ of the standard deviation, reaching less
than 0.1 MeV. Since during the evolution, the walkers at successive
steps should correlate, and thus the above uncertainty should be
under-estimated. There should be more precise estimate of uncertainty, such as the Jackknife method. Is the uncertainty really small, so that the quoted values have no errors? }\\

{\bf Our reply:} We thank the referee again for this constructive comment about the estimate of uncertainty. Since the DMC evolution is a Markov chain process, the values of adjacent steps are sequentially correlated, thus we should really consider their correlations when estimating the statistical uncertainty. To do this, we divide the steps into blocks and calculate the block averages. When the block size is taken large enough, the averages become uncorrelated and the uncertainty becomes independent of the block size.\\

After calculation, we find the average values have become uncorrelated when taking the block size as 500 steps. So we divide the last 5000 steps (used to calculate the center value) into 10 blocks of size 500 steps. Using the Jackknife resampling method, the uncertainty turns out to be less than 1 MeV. Take $\Omega^-(sss)$ as an example, the uncertainty is 0.3 MeV, which is about one order larger than the previous naive uncertainty estimation 0.04 MeV without considering the correlation.\\

In the new version of the manuscript, we make changes in  \cref{Jackknife}, \cref{uncertainty}, \cref{JackknifeSummary} and \cref{app_uncertainty}.\\





{\bf Comment: }\textit{ In the first paragraph of page 6, meaning of ``the confinement is proportional to the perimeter of the triangle
connecting three quarks'' is hard to understand.}\\

{\bf Our reply:} The meaning of this sentence is ``the confinement potential is proportional to the length of the perimeter of the triangle connecting three quarks''. This is because the two-body linear definition term is proportional to the distance between two quarks $r_{ij}$, namely, the length of one side of the triangle (if we connect the positions of 3 quarks into a triangle). The total confinement potential of a 3-quark system equals to the sum of the confinement potentials between any two of the three quarks. Besides, their coupling constants are the same. Thus the total confinement potential is proportional to the length of the perimeter $\sum_{i<j}r_{ij}$ of the triangle. \\

In the new version of the manuscript, we make a small change \cref{perimeter}.\\



